Effects of Quantum Communication in Large-Scale Networks at Minimum Latency

Quantum communication technology offers several advanced strategies. However, their practical use is often times not yet well understood. In this work we therefore analyze the concept of a futuristic large-scale robotic factory, where each robot has a computing unit associated to it. The computing unit assists the robot with large computational tasks that have to be performed in real-time. Each robot moves randomly in a vicinity of its computing unit, and in addition both the robot and the unit can change location. To minimize latency, the connection is assumed as optical wireless. Due to the mobility, a permanent optimal assignment of frequency bands is assumed to increase communication latency and is therefore ruled out. Under such assumptions, we compare the different capacity scaling of different types of such architectures, where the one is built utilizing quantum communication techniques, and the other based on conventional design methods.

==> code/05_scaling_two_ray_ground.tex <==
\subsection{Two-ray ground reflection loss model}

{\color{gray}
In the infinitely large grid, we also investigate the two strategies. One where all \ac{RCU} pairs communicate on a single wide band spanning the whole bandwidth. And one where each \ac{RCU} pair communicates on specific band.
}


\subsubsection{Bandwidth splitting strategy with finite grid of size $K$}
The power loss due to the two-ray model doesn't affect the communication capacities. The only noise that is present in this case is the constant background noise.

%BBAND SHARING STRATEGY with finite grid
\subsubsection{Band sharing strategy with finite gird of size $K$}

Similarly to previous case, we compute capacities for the factory, with finite \ac{RCU} pairs but two-ray loss power model. We set the distance between the nodes to $d=1$.

\begin{align}
    \tau &= 0.9\\
    b &= B\\
    n &= 10^{16}\\
    \nu(K) &= n
\end{align}

\begin{figure}[H]
    \centering
    \input{plots/sharing}
    \caption{plot}
    \label{fig:Burst_infinite_E_Buffers_higher_rate}
    
\end{figure}


\subsubsection{Comparison of the bandwidth splitting and bandwidth sharing strategies}


%BAND SHARING STRATEGY INFINITE GRID
\subsubsection{Bandwidth sharing strategy for the infinitely big grid}

The transmission power, baud rates and the noise levels in this scenario are defined by the following formulas:
\begin{align}
    b &= B \\
    \nu(d) &= \frac{n(d)}{d^4} \cdot C
\end{align}

where $C=6.03$ according to the formula in the \ref{eqn:ground_effect}.

\begin{figure}[H]
\centering
\begin{gnuplot}[terminal=cairolatex, terminaloptions={size 9cm, 6cm}]
    load 'gnuplot/functions.plt'
    load 'gnuplot/constants.plt'
    
    sigma = 1e5
    N(d) = sigma * d**2
    tau = 0.9
    b(d) =  BANDWIDTH_COM
    NU(d) = CONST_C * N(d)/(d**4)
    
    set xrange [1e1:1e5]
    unset yrange
    
    set logscale y
    set logscale x
    
    set xlabel "$d$"
    set ylabel "$bits/second$"
    
    # HERE IMPROVE RENDER QUALITY 
    set samples 100,100

    
    plot real(C_E(b(x), tau, N(x),   NU(x))) title "$C_{EA}$",\
          C_OJDR(b(x),  tau, N(x),   NU(x)) title "$C_{OJDR}$",\
          C_OSSR(b(x),  tau, N(x),   NU(x)) title "$C_{OSSR}$"

\end{gnuplot}
\caption{Communication capacities where all \ac{RCU} pairs communicate on the same wide band. With increasing density (falling $d$)}
\label{fig:infinite_grid_1}
\end{figure}


\subsubsection{Bandwidth splitting strategy within an infinite grid}

The bandwidth splitting strategy does not work in a case with infinite communicating nodes in an infinite grid because the baud rates would approach 0 with infinite participants.

In a specific case of relatively spatially stationary \ac{RCU} pairs one valid strategy would be to assign the bands to the \ac{RCU} pairs that are sufficiently far apart. Stationarity would rule out coordination and with band reuse the pairs would achieve a non-zero capacity.

==> rendered_plots/01_results/results_mmimo.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(4800.00,2260.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(616,764){\makebox(0,0)[r]{\strut{}$10^{8}$}}%
      \csname LTb\endcsname%%
      \put(616,1502){\makebox(0,0)[r]{\strut{}$10^{9}$}}%
      \csname LTb\endcsname%%
      \put(616,2239){\makebox(0,0)[r]{\strut{}$10^{10}$}}%
      \csname LTb\endcsname%%
      \put(717,525){\makebox(0,0){\strut{}$10^{0}$}}%
      \csname LTb\endcsname%%
      \put(1235,525){\makebox(0,0){\strut{}$10^{1}$}}%
      \csname LTb\endcsname%%
      \put(1752,525){\makebox(0,0){\strut{}$10^{2}$}}%
      \csname LTb\endcsname%%
      \put(2270,525){\makebox(0,0){\strut{}$10^{3}$}}%
      \csname LTb\endcsname%%
      \put(2788,525){\makebox(0,0){\strut{}$10^{4}$}}%
      \csname LTb\endcsname%%
      \put(3305,525){\makebox(0,0){\strut{}$10^{5}$}}%
      \csname LTb\endcsname%%
      \put(3823,525){\makebox(0,0){\strut{}$10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(17,1501){\rotatebox{-270}{\makebox(0,0){\strut{}$bps$}}}%
      \csname LTb\endcsname%%
      \put(2270,167){\makebox(0,0){\strut{}Number of link subdivisions}}%
      \csname LTb\endcsname%%
      \put(4390,1798){\makebox(0,0)[r]{\strut{}$C^{C}_{E}$}}%
      \csname LTb\endcsname%%
      \put(4390,1364){\makebox(0,0)[r]{\strut{}$C^{C}_{J}$}}%
      \csname LTb\endcsname%%
      \put(4390,930){\makebox(0,0)[r]{\strut{}$C^{C}_{S}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={240.00bp},height={113.00bp}]{rendered_plots/01_results/results_mmimo_p.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> rendered_plots/mMIMO/mmimo_cdma_ofdm.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(4800.00,2820.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(855,1764){\makebox(0,0)[r]{\strut{}$10^{0}$}}%
      \csname LTb\endcsname%%
      \put(855,1932){\makebox(0,0)[r]{\strut{}$10^{2}$}}%
      \csname LTb\endcsname%%
      \put(855,2100){\makebox(0,0)[r]{\strut{}$10^{4}$}}%
      \csname LTb\endcsname%%
      \put(855,2267){\makebox(0,0)[r]{\strut{}$10^{6}$}}%
      \csname LTb\endcsname%%
      \put(855,2435){\makebox(0,0)[r]{\strut{}$10^{8}$}}%
      \csname LTb\endcsname%%
      \put(956,1440){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1407,1440){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1858,1440){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2310,1440){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2761,1440){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(357,2099){\rotatebox{-270}{\makebox(0,0){\strut{}$bps$}}}%
      \csname LTb\endcsname%%
      \put(4217,2383){\makebox(0,0)[r]{\strut{}$C^{C+o}_{E}$}}%
      \csname LTb\endcsname%%
      \put(4217,2111){\makebox(0,0)[r]{\strut{}$C^{C+o}_{J}$}}%
      \csname LTb\endcsname%%
      \put(4217,1839){\makebox(0,0)[r]{\strut{}$C^{C+o}_{S}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(855,802){\makebox(0,0)[r]{\strut{}$10^{0}$}}%
      \csname LTb\endcsname%%
      \put(855,1236){\makebox(0,0)[r]{\strut{}$10^{1}$}}%
      \csname LTb\endcsname%%
      \put(956,431){\makebox(0,0){\strut{}$10^{0} $}}%
      \csname LTb\endcsname%%
      \put(1407,431){\makebox(0,0){\strut{}$10^{2} $}}%
      \csname LTb\endcsname%%
      \put(1858,431){\makebox(0,0){\strut{}$10^{4} $}}%
      \csname LTb\endcsname%%
      \put(2310,431){\makebox(0,0){\strut{}$10^{6} $}}%
      \csname LTb\endcsname%%
      \put(2761,431){\makebox(0,0){\strut{}$10^{8} $}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(477,1105){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(1971,191){\makebox(0,0){\strut{}$s$}}%
      \csname LTb\endcsname%%
      \put(4318,1403){\makebox(0,0)[r]{\strut{}${C^{C+o}_{E}}/{C^{C+o}_{S}}$}}%
      \csname LTb\endcsname%%
      \put(4318,1131){\makebox(0,0)[r]{\strut{}${C^{C+o}_{J}}/{C^{C+o}_{S}}$}}%
      \csname LTb\endcsname%%
      \put(4318,859){\makebox(0,0)[r]{\strut{}${C^{C+o}_{E}}/{C^{C+o}_{J}}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={240.00bp},height={141.00bp}]{rendered_plots/mMIMO/mmimo_cdma_ofdm_p.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> rendered_plots/mMIMO/mmimo_ofdm_ofdm.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(4800.00,2820.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(855,1764){\makebox(0,0)[r]{\strut{}$10^{0}$}}%
      \csname LTb\endcsname%%
      \put(855,1932){\makebox(0,0)[r]{\strut{}$10^{2}$}}%
      \csname LTb\endcsname%%
      \put(855,2100){\makebox(0,0)[r]{\strut{}$10^{4}$}}%
      \csname LTb\endcsname%%
      \put(855,2267){\makebox(0,0)[r]{\strut{}$10^{6}$}}%
      \csname LTb\endcsname%%
      \put(855,2435){\makebox(0,0)[r]{\strut{}$10^{8}$}}%
      \csname LTb\endcsname%%
      \put(956,1440){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1407,1440){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(1858,1440){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2310,1440){\makebox(0,0){\strut{}}}%
      \csname LTb\endcsname%%
      \put(2761,1440){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(357,2099){\rotatebox{-270}{\makebox(0,0){\strut{}$bps$}}}%
      \csname LTb\endcsname%%
      \put(4217,2383){\makebox(0,0)[r]{\strut{}$C^{O+o}_{E}$}}%
      \csname LTb\endcsname%%
      \put(4217,2111){\makebox(0,0)[r]{\strut{}$C^{O+o}_{J}$}}%
      \csname LTb\endcsname%%
      \put(4217,1839){\makebox(0,0)[r]{\strut{}$C^{O+o}_{S}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(855,802){\makebox(0,0)[r]{\strut{}$10^{0}$}}%
      \csname LTb\endcsname%%
      \put(855,1236){\makebox(0,0)[r]{\strut{}$10^{1}$}}%
      \csname LTb\endcsname%%
      \put(956,431){\makebox(0,0){\strut{}$10^{0} $}}%
      \csname LTb\endcsname%%
      \put(1407,431){\makebox(0,0){\strut{}$10^{2} $}}%
      \csname LTb\endcsname%%
      \put(1858,431){\makebox(0,0){\strut{}$10^{4} $}}%
      \csname LTb\endcsname%%
      \put(2310,431){\makebox(0,0){\strut{}$10^{6} $}}%
      \csname LTb\endcsname%%
      \put(2761,431){\makebox(0,0){\strut{}$10^{8} $}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(477,1105){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \csname LTb\endcsname%%
      \put(1971,191){\makebox(0,0){\strut{}$s$}}%
      \csname LTb\endcsname%%
      \put(4318,1403){\makebox(0,0)[r]{\strut{}${C^{O+o}_{E}}/{C^{O+o}_{S}}$}}%
      \csname LTb\endcsname%%
      \put(4318,1131){\makebox(0,0)[r]{\strut{}${C^{O+o}_{J}}/{C^{O+o}_{S}}$}}%
      \csname LTb\endcsname%%
      \put(4318,859){\makebox(0,0)[r]{\strut{}${C^{O+o}_{E}}/{C^{O+o}_{J}}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={240.00bp},height={141.00bp}]{rendered_plots/mMIMO/mmimo_ofdm_ofdm_p.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> v2_05_scaling_two_ray_ground.tex <==
\subsection{Capacity scaling with two-ray loss model}

\subsection{Orthogonal Frequency Division Multiplexing with finitely big factory}

The power loss due to the two-ray model doesn't affect the communication capacities when using the \ac{OFDM}. The only noise that is present in this case is the constant background noise. Again the capacity reduction occurs due to the narrowing of the bands. So the capacities scale in the same way they scale in the OFDM case with free space loss shown in figure \ref{fig:ofdm_free_space}.

\subsubsection{Code Division Multiple Access communication with finitely big factory size}

Similarly to previous case, we compute capacities for the factory, with finite \ac{RCU} pairs but two-ray loss power model. We set the distance between the nodes to $d=1$.
%
%
%\begin{figure}[H]
%    \centering
%    \input{plots/comparing_results}
%    \caption{Single link CDMA capacities in a factory where two-ray signal loss is observed. Plotted are capacity scaling with the parameters: $B=10^{12}$ Hz, $n=10^{11}$ , $\tau=0.99$, $\nu_b=10^3$. }
%    \label{fig:cdma_ground_loss}
%\end{figure}
%
%
%\subsection{Comparing OFDM and CDMA capacity scaling in the factory with two-ray loss}
%
When ground effect signal loss is observed the multiplication of the capacity, when switching from the OFDM to CDMA, is also increasing as the factory grows. Bigger multiplication factors are expected, since the bigger signal loss effectively reduces the amount of noise \ac{RCU} has to withstand when using CDMA based communication protocols. But in the case of OFDM the communication is still limited by the individual band widths. The multiplication scaling implies that, the bigger factory becomes, the more improvement in individual capacities one can expect using joint detector receiver design and even more when entanglement assistance is used. 

%\begin{figure}[H]
%    \centering
%    \input{plots/comparing}
%    \caption{Capacity multiplication scaling with parameters from the figures \ref{fig:cdma_ground_loss} ($B=10^{12}$ Hz, $N_{P}=10^{11}$ , $\tau=0.99$, $\nu_b=10^3$).}
%    \label{fig:sharing_2}
%\end{figure}
%
%\begin{figure}[H]
%    \centering
%    \input{plots/cdma}
%    \caption{Capacity multiplication scaling with parameters from the figures \ref{fig:cdma_ground_loss} ($B=10^{12}$ Hz, $N_{P}=10^{11}$ , $\tau=0.99$, $\nu_b=10^3$).}
%    \label{fig:sharing_2}
%\end{figure}


\subsubsection{CDMA communication capacities in an infinitely large factory with two-ray loss}

The baudrate and attenuation from capacity parameters $(b,\tau, n, \nu)$ were defined similarly as in previous cases: $b=B$, $\tau=0.99$. Emission power was defined as constant in power per area $\sigma=10^2$. Each \ac{RCU} was given $n=\sigma / d^2$ power, where $d$ again denotes distance between the communicating pairs.

The interfering noise was calculated using the following formula:

\begin{align}
    \nu(n,d,K) &= 4 \cdot
    \sum_{x=1}^{K} \sum_{y=1}^K
    \frac{n}{((dx)^2+(dy)^2)^2} 
    \Big)\\
    \nu(n,d) &= \lim_{K\to \infty} \nu(n,d,K)\\
    \nu(n,d) &= \frac{n}{d^4} \Big[4 X + 4\frac{\pi^4}{90}\Big] = \frac{n}{d^4}\cdot C
\end{align}

With $X$ representing the value of double summation term, which converges ($X\approx 0.42437$). And $C$ representing whole value of the square brackets $C\approx 6.03$.

%\begin{figure}[H]
%\centering
%\begin{gnuplot}[terminal=cairolatex, terminaloptions={size 9cm, 6cm}]
%    load 'gnuplot/functions.plt'
%    load 'gnuplot/constants.plt'
%    
%    power = POWER_COM
%    bandwidth = BANDWIDTH_COM
%    N(d) = power
%    tau = 0.99
%    b(d) =  BANDWIDTH_COM
%    NU(d) = CONST_C * N(d)/(d**4)
%    bandwidth = BANDWIDTH_COM
%    
%    set xrange [K_MIN:K_MAX]
%    unset yrange
%    
%    set logscale y
%    set logscale x
%    
%    set xlabel "$d$"
%    set ylabel "$bits/second$"
%    
%    # HERE IMPROVE RENDER QUALITY
%    set samples 100,100
%    
%    
%    set key right bottom
%    tau = 0.99 
%    plot C_E(b(x), tau, power,   NU(x)) title "$C_{E}$" ls 1,\
%            C_OJDR(b(x),  tau, power,   NU(x)) title "$C_{J}$" ls 2,\
%            C_OSSR(b(x),  tau, power,   NU(x)) title "$C_{S}$" ls 3
%\end{gnuplot}
%\caption{ \ac{CDMA} capacity scaling in an infinitely large factory with two-ray model loss. The following parameters were fixed: $\sigma=10^3$ , $\tau=0.99$. Again quantum techniques offer better rates than classical ones.}
%\label{fig:infinite_grid_1}
%\end{figure}


\subsubsection{OFDM communication capacity in an infinitely large grid}

The OFDM communication scheme does not work in a case with infinite communicating nodes in an infinite grid because the baud rates vanish with infinite participants.

In a specific case of relatively spatially stationary \ac{RCU} pairs one valid strategy would be to assign the bands to the \ac{RCU} pairs that are sufficiently far apart. Stationarity would rule out coordination and with band reuse the pairs would achieve a non-zero capacity. 
